Understanding Real-World AI Planning Domains: A Conceptual Framework

Planning is a pivotal ability of any intelligent system being developed for real-world applications. AI planning is concerned with researching and developing planning systems that automatically compute plans that satisfy some user objective. Identifying and understanding the relevant and realistic aspects that characterise real-world application domains are crucial to the development of AI planning systems. This provides guidance to knowledge engineers and software engineers in the process of designing, identifying, and categorising resources required for the development process. To the best of our knowledge, such support does not exist. We address this research gap by developing a conceptual framework that identifies and categorises the aspects of real-world planning domains in varying levels of granularity. Our framework provides not only a common terminology but also a comprehensive overview of a broad range of planning aspects exemplified using the domain of sustainable buildings as a prominent application domain of AI planning. The framework has the potential to impact the design, development, and applicability of AI planning systems in real-world application domains.

==> usecase.tex <==
\section{Use Case: Sustainable Buildings}
%EA: The first subsection will be moved to the preliminaries and the examples of the second subsection will be integrated in Section 4 where we explain the hierarchy.
\subsection{Overview of Sustainable Buildings Domain}
We illustrate the realistic-aspects hierarchy using the sustainable buildings domain. The operation of these buildings depends on the effectiveness and efficiency of their Building Management Systems (BMSs), which are computer-and-device-based control systems aiming at monitoring, storing, and communicating data, and supervising, controlling, and automating the various systems in these buildings~\cite{levermore2000building}. Examples of devices in sustainable buildings include sensors (e.g., position and temperature sensors), and actuators (e.g., switches on ceiling lamps). Systems in these buildings can include Heating, Ventilation, Air conditioning (HVAC), lighting, access control, security, electrical, and other interrelated systems. The main objectives of BMSs include increasing safety, improving people's productivity, cutting energy consumption; hence preserving finite resources, using non-carbon sources when possible to lower the CO2 footprint, and lowering the costs of consumers and businesses while preserving users' comfort~\cite{georgievski2017planning,fiorini2019energy}. This is especially true for buildings that are connected to a smart grid, which makes it possible to include renewable sources and provides dynamic pricing and energy offers coming from competing providers~\cite{georgievski2015coordinating}. The advent of the Internet of Things (IoT) offers significant opportunities to improve the limited control capabilities offered by current building management systems, such as the reactive control and feedback mechanisms~\cite{georgievski2017planning,georgievski2023babtp}.

\subsection{Realistic-Aspects Hierarchy Illustrated on the Sustainable Buildings Domain}
The process of engineering knowledge in this domain for AI planning should consider various realistic aspects characterising this domain. The planning domain knowledge should reflect the hard goals of the BMS whether these goals are qualitative or quantitative. For example, one qualitative hard goal of the BMS could be to improve the comfort of the building's occupants, while a quantitative hard goal could be to minimise the operation costs of the building to a certain value per year. Goals can be also expressed as preferences. For example, the BMS might have the soft goal of keeping the floors clean. This goal can be a subgoal of the goal of increasing occupants' comfort. The latter can have another subgoal, such as the quantitative subgoal of maintaining the office temperature between 15-20$^{\circ}$. Moreover, some goals can be defined as optimisation goal, which requires finding optimal plans given the current conditions of the building. For example, according to the market prices, the amount of stored energy, and the weather forecast, the goal could be to find a plan that optimises the energy consumption of the building. Goals can be also expressed as satisfaction goals. For example, given the aforementioned building conditions, the goal is to compute plans that do not exceed a certain threshold of energy consumption. Additionally, the goals of the BMS could have specific strict ordering constraints that define the importance of or the criticality of achieving one goal compared to other goals. In this domain, some goals should have a strict total order. For example, the goal of having a safe environment in the building must not have a higher priority than the goal of cutting energy consumption or having a comfortable environment. Some other goals can have unrestricted order of their criticality. For example, the goals of minimising energy consumption and maintaining a comfortable work environment can have the same importance.

In addition to the goals, the planning domain model for sustainable buildings should contain the different components/agents that exist in the building. These include occupants of the building and automated components. The latter can be, for example, devices, such as actuators, sensors, and batteries to store energy, and robots used for teleconferencing and cleaning. Components also include application services that can be commercial, such as Microsoft PowerPoint, or have a specific purpose, such as application services to control the desired thresholds of lighting and heating. Finally, components can be information services. For example, an information service to get the weather forecast.

Agents in sustainable buildings perform operations either for the purpose of achieving goals or as part of their regular activities. For example, an actuator that controls the blinds' movement in the office could close the blinds to achieve the goal of keeping the light intensity at a certain level. However, a person turning on her/his PC could be an operation that is performed not for the purpose of satisfying a planning goal but for the purpose of working on the PC.

Operations performed by agents have spatial properties that relate them and the agent performing them to one another and with the space. The first type of spatial properties relates to human operations. For example, an occupant moves from the corridor to the office. The second type is related to automated components. For example, the operation of the actuator that controls the blinds has a spatial extension. These spatial properties can be represented abstractly without considering any geometrical or physical laws. An example of this is assuming that an occupant movement from the corridor to the office happens or the battery storing the energy generated from solar panels happens instantaneously. The other representation is the pure representation that considers the spatial arrangement of the building and sometimes the spatiotemporal properties. This means that representing the movement of an occupant requires considering the time required for the movement and the spatial arrangement of the corridor and the office.

In addition to the spatial arrangement, operations have temporal properties that relate them to one another with respect to time. The domain model should be able to reflect the different ways of representing the relation between these two operations. In particular, we should be able to model the operation that spans a period of time or the start and end of each operation. In the first case, the operation of storing energy coming from solar panels in batteries should precede the operation of operating the air conditioner using local energy stored in batteries. In the second case, the start of the operating the air conditioner operation should follow the end of the storing energy in batteries operation. While some operations must have a strict total temporal ordering, other operations can be unordered, partially ordered, or required to be done concurrently. For example, in the previous example, we can have a strict ordering between the operation of storing energy and the operation of operating the air conditioner, or we can have a flexible order, as long as the battery has enough energy. 

Some constraints can come from the building regulations, policies, or standards and they aim at improving, for example, the occupants' health, effectiveness, and safety. For example, the operations of turning lights on/off and controlling the intensity of the lights in the office can follow some standards for lighting in indoor work places~\cite{georgievski2017planning}. Some other constraints are defined with respect to the spatial properties of the agents. For example, during the COVID-19 pandemic, regulations are defined to restrict the distance between two persons working in the same workplace.

Other types of constraints on the operations performed in sustainable buildings could be of economical nature. An example of these kinds of constraints can be a constraint on the maximum energy consumption induced as a result of performing a specific operation, i.e., the cost of performing a specific operation.

In the sustainable buildings domain, like most of the real-world planning domains, there are different ways of achieving the same operation. For example, increasing the light intensity in the office can be done by either pulling the curtains up or by turning on the lights.

Operations, such as storing solar energy in batteries, should be planned for while considering several types of uncertainty. The uncertainty can be caused by sources external to the agent/components executing the operation. For example, weather conditions, which are considered a regular changing source of uncertainty, can affect the amount of energy stored in the batteries. Another source of uncertainty can be internal. For example, a malfunction in a battery is considered a random internal source of uncertainty that can affect the amount of locally stored energy. Other sources of uncertainty include the energy demand and market prices~\cite{fiorini2019energy,fiorini2020predictive}. The existence of uncertainty can lead to partial observability of the environment's current condition. For example, an internal malfunction in the sensors responsible for detecting whether the person is working on his/her PC can lead to partial knowledge about the current conditions of the environment. Another consequence of the uncertainty existence is having unexpected or different possible outcomes of operation effects and costs. For example, turning on the radiator to heat the office might lead to the radiator not being turned on due to internal malfunction. Additionally, turning on the radiator might have costs that are hard to predefine with certainty. The reason for this could be not having enough locally stored energy due to unexpected weather conditions. This necessitates buying energy, which incurs costs that depend on the market prices. When we either have knowledge about the probability distribution of the operation outcomes or we can statically infer it, we are dealing with a domain that contains risk. However, we have partial or no knowledge about the probability distribution, we are dealing we a domain that is uncertain.

When dealing with domains that involve risk and uncertainty, the domain knowledge should also reflect the risk attitude and trust of the users in the autonomous system. For example, assume that the building can get its electricity from two different sources; either from stored electricity generated locally by renewable resources or from electric utilities with varying prices and energy offers. The choice of whether to consume locally generated electricity or the purchasing it from outside sources should be made under uncertainty about the future market prices and the future weather forecast. For example, let us assume that the building management system has the following information. There is a high probability of having a cloudy next day, i.e., no energy can be stored in the batteries and a small probability of having a sunny day. However, there is information about the day-ahead prices offered by different providers. The building management system might follow a risk-seeking attitude and decides not to purchase energy and rely on the possibility of having a sunny day, i.e., using solar energy.

%later: add an example about trust
% decide later whether to also add examples related to domain construction


